DIMSpan - Transactional Frequent Subgraph Mining with Distributed In-Memory Dataflow Systems

Transactional frequent subgraph mining identifies frequent subgraphs in a collection of graphs. This research problem has wide applicability and increasingly requires higher scalability over single machine solutions to address the needs of Big Data use cases. We introduce DIMSpan, an advanced approach to frequent subgraph mining that utilizes the features provided by distributed in-memory dataflow systems such as Apache Spark or Apache Flink. It determines the complete set of frequent subgraphs from arbitrary string-labeled directed multigraphs as they occur in social, business and knowledge networks. DIMSpan is optimized to runtime and minimal network traffic but memory-aware. An extensive performance evaluation on large graph collections shows the scalability of DIMSpan and the effectiveness of its pruning and optimization techniques.

==> 211_binary.tex <==
\begin{table}

\raggedright

\begin{tabular}{llll}
\textbf{Transf.} & \textbf{Signature}\hspace{5mm} & \textbf{Constraints} \\
Cross     & $I_1 \subseteq A; I_2 \subseteq B$ & $O = I_1 \times I_2$     \\
Union     & $I_1, I_2 \subseteq A$ & $O = I_1 \cup I_2$     \\
\end{tabular}
\vspace{2mm}

(I/O : input/output datasets, A..D : domains, W : worker threads)\\
\vspace{2mm}


\caption{Example Unary Dataflow Tranformations}
\label{tab:binary}

\end{table}


==> 311_preprocessing.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\REQUIRE{$\mathcal{G}_{S/S}, s_{min}$}
\STATE $f_{min} \leftarrow \left| \mathcal{G}_{S/S} \right| * s_{min}$
\STATE $\delta_v \leftarrow frequentVertexLabels(\mathcal{G}_{S/S}, f_{min})$
\STATE \textbf{broadcast}($\delta_v$)
\STATE $\mathcal{G}_{I/S} \leftarrow \mathcal{G}_{S/S}.\textbf{map}(encodeAndFilterVertices)$
\STATE $\delta_e \leftarrow frequentEdgeLabels(\mathcal{G}_{I/S}, f_{min})$
\STATE \textbf{broadcast}($\delta_e$)
\STATE $\mathcal{G} \leftarrow \mathcal{G}_{I/S}.\textbf{map}(encodeAndFilterEdges)$
\STATE $\mathcal{F} \leftarrow FSM(\mathcal{G}, f_{min})$
\STATE $\mathcal{F}_{S/S} \leftarrow  \mathcal{F}.\textbf{map}(decode)$
\RETURN $\mathcal{F}_{S/S}$

\end{algorithmic}
\caption{Pre- and postprocessing dataflow.}
\label{alg:pre}
\end{algorithm}


==> 331_complexity.tex <==
\begin{table}

\begin{subtable}{0.48\textwidth}
\begin{tabular}{lc|cccc}
 & & combine & counting & reduce & globalization\ \\
&  & input & network & input & network\ \\
Time 
& comp.
& $g \times p$
& $w \times p$
& $w \times p$
& $w \times f$
\\
\hline
Without
&0
&$v$
&$v$
&$v$
&$v$
\\
Map
&$g \times p$
&$v/c$
&$v/c$
&$v/c$
&$v/c$
\\
Combine
&$w \times p$
&$v$
&$v/c$
&$v/c$
&$v/c$
\\
Filter
&$f$
&$v$
&$v$
&$v$
&$v/c$
\\
\end{tabular}
\caption{Varying compression time.}
\end{subtable}

\begin{subtable}{0.48\textwidth}
\begin{tabular}{lc|cccc}
 & & combine & counting & reduce & globalization\ \\
&  & input & network & input & network\ \\
Time 
& comp.
& $g \times v$
& $w \times v$
& $w \times v$
& $w \times v$
\\
\hline
Map
&$g \times p$
&$p - p'$
&$p - p'$
&$p - p'$
&$f$
\\
Combine
&$w \times p$
&$p$
&$p - p'$
&$p - p'$
&$f$
\\
Filter
&$f$
&$p$
&$p$
&$p$
&$f$
\\
\end{tabular}
\caption{Varying validation time.}
\end{subtable}

\begin{subtable}{0.48\textwidth}
\begin{tabular}{clcl}
$g$ & number of graphs            & $w$ & number of workers \\
$p$ & number of patterns          & $v$ & average volume per pattern \\
$f$ & number of frequent patterns & $c$ & compression rate \\
$p'$ & number of false positives \\

\end{tabular}
\end{subtable}

\caption{Compressionb \& Validation}
\label{tab:steps}
\end{table}


==> 40_implementation.tex <==



\section{Implementation}
\label{sec:impl}
Our approach to distributed FSM was implemented as an extension of the \textsc{Gradoop} framework \cite{junghanns2016epgm}, a 3rd party library of the distributed dataflow framework Apache Flink \cite{carbone2015apache}. In the following, we will briefly introduce \textsc{Gradoop} and Flink and provide implementation details.

\input{41_gradoop}

\subsection{Apache Flink}

\input{43_structures}


\subsection{Preprocessing}
\subsection{Distributed Iterative Mining}


==> 41_gradoop.tex <==
\subsection{\textsc{Gradoop} Framework}

\textsc{Gradoop} \cite{junghanns2016epgm} is a system for declarative graph analytics. It allows the combination of multiple graph operators and graph mining algorithms in a single analytical program. To enable distributed execution of analytical programs on shared nothing clusters, \textsc{Gradoop}'s graph representation is mapped to the dataset abstraction and operators as well as algorithms are implemented using Flink's transformations. The source code of \textsc{Gradoop} is available online under the GPL license\footnote{\url{www.gradoop.com}}.

A \textsc{Gradoop} program can be represented by a directed acyclic graph (DAG) where vertices are graphs or graph collections and edges are operators or algorithms. Besides general-purpose operators (e.g., the union of two graph collections) the framework provides a generic \textit{call} operator and fitting Java interfaces to make arbitrary graph mining algorithms applicable in \textsc{Gradoop} analytical programs. Our approach to distributed FSM was designed to be applicable with the call operator. However, we also provide a standalone program\footnote{\url{github...}} to use our implementation without the framework. In contrast to other FSM implementations, we support directed or undirected multigraphs without arbitrary string labels as input and require not upfront integer-relabeling or sorting.


==> 43_structures.tex <==

\subsection{Data Structures}
\label{sec:model}
We performed preliminary experiments to find data structures that are space efficient, show a good performance for lexicographic comparison (branch restriction, false positive validation) and equality testing (counting) and can be fast serialized and deserialized between Flink transformations. Therefore, we evaluated the performance of Java objects, strings, byte arrays, nested integer arrays and multiplexed integer arrays. We found out that multiplexed integer arrays meet all of the three criteria best, in particular with regard to the fast but effective compression techniques available for integer arrays \cite{lemire2015decoding}.

The main data structures used in our approach are graphs, patterns and their embeddings. We use integer arrays of length $6 \times k$ to represent $k$-edge patterns and graphs, in particular $G/P = \langle v^1_a, v^1_b, l^1_a, d^1, l^1_e, l^1_b,..,v^k_a, v^k_b, l^k_a, d^k, l^k_e, l^k_b \rangle$. In graphs, edge are already stored in their minimal traversal direction according to gSpan lexicographic order.


==> 51_mrflow.tex <==
% \subsection{Comparison to Dataflow-based Approaches}


 
% The pioneer approach I-FSM follows a subgraph-centric BFS pattern growth approach and requires two MRMap-Reduce phases, in the following just called \textit{phases}, per iteration. For better understanding, we start with the second phase. The input of the second phase are $k+1$-edge subgraphs and in its map-step a (not further specified) canonical label is calculated for each subgraph. In the reduce step, subgraph-label pairs are shuffled, label frequency is counted and subgraphs with frequent labels are filtered. In the first phase, last iteration's subgraphs with frequent labels are shuffled by graph id, graphs are (partially) recovered by a union of all $k-edge$ subgraphs and all $k+1$-edge connected subgraphs are calculated to become input of the second phase. 
% 
% 
% 
% In \cite{lu2013efficiently} Lu et al. propose MRFSE, and advanced BFS pattern growth approach with only $k_{max}$ map-reduce phases. For each $k$, patterns and embeddings are read from FS and embeddings of frequent patterns are extended in the map step. Here, gSpan minimum DFS code is used for canonical labeling. Duplicate validation is also done in the map step, in particular by enumerating all grown labels per unique embedding to determine the canonical one. In the reduce step, solely patterns are counted and filtered. In contrast to \cite{hill2012iterative} subgraph information (pattern and embeddings) are written only once to disk and only patterns need to be shuffled among workers. A further notable performance gain is achieved by applying a partitioning strategy.
% 
% FSM-H \cite{bhuiyan2015iterative} is another iterative MapReduce based approach proposed by Bhuiyan and Hasan. FSM-H follows an apriori approach and is thus facing the problems of candidate generation and subgraph isomorphism testing. In an experimental evaluation, FSM-H shows a better performance than \cite{hill2012iterative} on molecular datasets with a high threshold, i.e., a low number of frequent patterns. The authors see the main reason in reduced network load caused by only shuffling patterns but not embeddings. Further on, FSM-H requires no upfront specification of the maximum number of iterations. Additionally, there exists an approach to approximate FSM based on MapReduce \cite{aridhi2014novel}.
% 
% \textbf{Subgraph Relabeling vs. False Positive Validation}: In MapReduce based approaches to pattern growth FSM different strategies are applied to generate and validate canonical labels of patterns. In \cite{hill2012iterative} canonical labels are completely recalculated for every embedding of a pattern. In \cite{lu2013efficiently}, canonical labels are generated by parent extension and validated by selecting the canonical one out of all labels generated for a distinct embedding. As canonical labeling contains the graph isomorphism problem \cite{schoning1988graph}, the first one is obviously ineffective. The second approach just hides the problem in enumerating all labels generated for each embedding of pattern. Consequently, both approaches face the graph isomorphism problem during the label generation process. In the comparison of \cite{worlein2005quantitative} the authors reported that label generation has more impact on the total runtime than validating false positives after counting them. As we could confirm this in own experiments, we apply label validation after counting (See Section \ref{sec:validation}).

